First lattice calculation of radiative leptonic decay rates of pseudoscalar mesons

We present a non-perturbative lattice calculation of the form factors which contribute to the amplitudes for the radiative decays $P\to \ell \bar \nu_\ell \gamma$, where $P$ is a pseudoscalar meson and $\ell$ is a charged lepton. Together with the non-perturbative determination of the corrections to the processes $P\to \ell \bar \nu_\ell$ due to the exchange of a virtual photon, this allows accurate predictions at $O(\alpha_{em})$ to be made for leptonic decay rates for pseudoscalar mesons ranging from the pion to the $D_s$ meson. We are able to separate unambiguously and non-pertubatively the point-like contribution, from the structure-dependent, infrared-safe, terms in the amplitude. The fully non-perturbative $O(a)$ improved calculation of the inclusive leptonic decay rates will lead to the determination of the corresponding Cabibbo-Kobayashi-Maskawa (CKM) matrix elements also at $O(\alpha_{em})$. Prospects for a precise evaluation of leptonic decay rates with emission of a hard photon are also very interesting, especially for the decays of heavy $D$ and $B$ mesons for which currently only model-dependent predictions are available to compare with existing experimental data.

==> Paper-Final Version/tabs/systematics_data_FA_Dphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_A \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_A $  & $\Delta_{F_A} $\\ \hline
0 &  0.11029 &  0.00885428 \\ \hline 
0.1 &  0.0988347 &  0.00740568 \\ \hline 
0.2 &  0.0887281 &  0.00727782 \\ \hline 
0.3 &  0.079585 &  0.00791868 \\ \hline 
0.4 &  0.0711547 &  0.0092365 \\ \hline 
0.5 &  0.063267 &  0.0111973 \\ \hline 
0.6 &  0.0558021 &  0.0137148 \\ \hline 
0.7 &  0.0486731 &  0.0166835 \\ \hline 
0.8 &  0.0418154 &  0.0200096 \\ \hline 
0.9 &  0.0351801 &  0.02362 \\ \hline 
1 &  0.0287293 &  0.027459 \\ \hline 
\end{tabular}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 0.907& 0.704& 0.491& 0.314& 0.187& 0.102& 0.049& 0.015& -0.006& -0.020\\ 
0.907& 1.000& 0.931& 0.776& 0.598& 0.439& 0.314& 0.223& 0.156& 0.108& 0.072\\ 
0.704& 0.931& 1.000& 0.948& 0.827& 0.688& 0.564& 0.465& 0.387& 0.327& 0.281\\ 
0.491& 0.776& 0.948& 1.000& 0.961& 0.875& 0.781& 0.697& 0.627& 0.570& 0.524\\ 
0.314& 0.598& 0.827& 0.961& 1.000& 0.974& 0.921& 0.863& 0.810& 0.764& 0.726\\ 
0.187& 0.439& 0.688& 0.875& 0.974& 1.000& 0.985& 0.954& 0.920& 0.888& 0.859\\ 
0.102& 0.314& 0.564& 0.781& 0.921& 0.985& 1.000& 0.991& 0.974& 0.953& 0.934\\ 
0.049& 0.223& 0.465& 0.697& 0.863& 0.954& 0.991& 1.000& 0.995& 0.985& 0.972\\ 
0.015& 0.156& 0.387& 0.627& 0.810& 0.920& 0.974& 0.995& 1.000& 0.997& 0.991\\ 
-0.006& 0.108& 0.327& 0.570& 0.764& 0.888& 0.953& 0.985& 0.997& 1.000& 0.998\\ 
-0.020& 0.072& 0.281& 0.524& 0.726& 0.859& 0.934& 0.972& 0.991& 0.998& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}


==> Paper-Final Version/tabs/systematics_data_FA_Dsphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_A \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_A $  & $\Delta_{F_A} $\\ \hline
0 &  0.09307 &  0.00598514 \\ \hline 
0.1 &  0.0849608 &  0.00486963 \\ \hline 
0.2 &  0.0776688 &  0.00422644 \\ \hline 
0.3 &  0.0709899 &  0.00389515 \\ \hline 
0.4 &  0.0647833 &  0.00400167 \\ \hline 
0.5 &  0.0589483 &  0.00469896 \\ \hline 
0.6 &  0.0534115 &  0.00595597 \\ \hline 
0.7 &  0.0481175 &  0.00763605 \\ \hline 
0.8 &  0.0430239 &  0.00962076 \\ \hline 
0.9 &  0.0380979 &  0.0118319 \\ \hline 
1 &  0.0333133 &  0.0142191 \\ \hline 
\end{tabular}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 0.959& 0.862& 0.725& 0.537& 0.338& 0.186& 0.091& 0.034& 0.001& -0.020\\ 
0.959& 1.000& 0.966& 0.861& 0.664& 0.423& 0.224& 0.091& 0.006& -0.048& -0.084\\ 
0.862& 0.966& 1.000& 0.957& 0.802& 0.569& 0.357& 0.206& 0.105& 0.037& -0.010\\ 
0.725& 0.861& 0.957& 1.000& 0.937& 0.768& 0.583& 0.437& 0.334& 0.261& 0.208\\ 
0.537& 0.664& 0.802& 0.937& 1.000& 0.942& 0.824& 0.713& 0.626& 0.561& 0.512\\ 
0.338& 0.423& 0.569& 0.768& 0.942& 1.000& 0.966& 0.906& 0.848& 0.802& 0.764\\ 
0.186& 0.224& 0.357& 0.583& 0.824& 0.966& 1.000& 0.984& 0.956& 0.928& 0.903\\ 
0.091& 0.091& 0.206& 0.437& 0.713& 0.906& 0.984& 1.000& 0.993& 0.979& 0.965\\ 
0.034& 0.006& 0.105& 0.334& 0.626& 0.848& 0.956& 0.993& 1.000& 0.996& 0.989\\ 
0.001& -0.048& 0.037& 0.261& 0.561& 0.802& 0.928& 0.979& 0.996& 1.000& 0.998\\ 
-0.020& -0.084& -0.010& 0.208& 0.512& 0.764& 0.903& 0.965& 0.989& 0.998& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}


==> Paper-Final Version/tabs/systematics_data_FA_Kphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_A \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_A $  & $\Delta_{F_A} $\\ \hline
0 &  0.0370382 &  0.00876335 \\ \hline 
0.1 &  0.0369171 &  0.00828189 \\ \hline 
0.2 &  0.0367961 &  0.00784116 \\ \hline 
0.3 &  0.0366751 &  0.00744839 \\ \hline 
0.4 &  0.0365541 &  0.00711155 \\ \hline 
0.5 &  0.0364331 &  0.00683889 \\ \hline 
0.6 &  0.0363121 &  0.00663833 \\ \hline 
0.7 &  0.0361911 &  0.00651654 \\ \hline 
0.8 &  0.0360701 &  0.00647795 \\ \hline 
0.9 &  0.0359491 &  0.00652404 \\ \hline 
1 &  0.035828 &  0.00665305 \\ \hline 
\end{tabular}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 0.998& 0.990& 0.975& 0.951& 0.916& 0.869& 0.808& 0.736& 0.654& 0.566\\ 
0.998& 1.000& 0.997& 0.988& 0.970& 0.941& 0.899& 0.845& 0.779& 0.703& 0.620\\ 
0.990& 0.997& 1.000& 0.997& 0.985& 0.963& 0.929& 0.883& 0.823& 0.753& 0.676\\ 
0.975& 0.988& 0.997& 1.000& 0.996& 0.982& 0.957& 0.918& 0.867& 0.805& 0.734\\ 
0.951& 0.970& 0.985& 0.996& 1.000& 0.995& 0.979& 0.950& 0.909& 0.855& 0.793\\ 
0.916& 0.941& 0.963& 0.982& 0.995& 1.000& 0.994& 0.976& 0.946& 0.902& 0.849\\ 
0.869& 0.899& 0.929& 0.957& 0.979& 0.994& 1.000& 0.994& 0.975& 0.943& 0.900\\ 
0.808& 0.845& 0.883& 0.918& 0.950& 0.976& 0.994& 1.000& 0.993& 0.974& 0.943\\ 
0.736& 0.779& 0.823& 0.867& 0.909& 0.946& 0.975& 0.993& 1.000& 0.994& 0.975\\ 
0.654& 0.703& 0.753& 0.805& 0.855& 0.902& 0.943& 0.974& 0.994& 1.000& 0.994\\ 
0.566& 0.620& 0.676& 0.734& 0.793& 0.849& 0.900& 0.943& 0.975& 0.994& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}


==> Paper-Final Version/tabs/systematics_data_FA_Piphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_A \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_A $  & $\Delta_{F_A} $\\ \hline
0 &  0.0104088 &  0.00262483 \\ \hline 
0.1 &  0.0104435 &  0.00260149 \\ \hline 
0.2 &  0.0104782 &  0.0025792 \\ \hline 
0.3 &  0.0105129 &  0.00255799 \\ \hline 
0.4 &  0.0105477 &  0.00253788 \\ \hline 
0.5 &  0.0105824 &  0.00251889 \\ \hline 
0.6 &  0.0106171 &  0.00250106 \\ \hline 
0.7 &  0.0106519 &  0.00248441 \\ \hline 
0.8 &  0.0106866 &  0.00246897 \\ \hline 
0.9 &  0.0107213 &  0.00245474 \\ \hline 
1 &  0.010756 &  0.00244177 \\ \hline 
\end{tabular}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 1.000& 0.999& 0.998& 0.997& 0.995& 0.992& 0.989& 0.986& 0.982& 0.977\\ 
1.000& 1.000& 1.000& 0.999& 0.998& 0.997& 0.995& 0.992& 0.989& 0.985& 0.981\\ 
0.999& 1.000& 1.000& 1.000& 0.999& 0.998& 0.996& 0.994& 0.992& 0.989& 0.985\\ 
0.998& 0.999& 1.000& 1.000& 1.000& 0.999& 0.998& 0.996& 0.994& 0.992& 0.988\\ 
0.997& 0.998& 0.999& 1.000& 1.000& 1.000& 0.999& 0.998& 0.996& 0.994& 0.991\\ 
0.995& 0.997& 0.998& 0.999& 1.000& 1.000& 1.000& 0.999& 0.998& 0.996& 0.994\\ 
0.992& 0.995& 0.996& 0.998& 0.999& 1.000& 1.000& 1.000& 0.999& 0.998& 0.996\\ 
0.989& 0.992& 0.994& 0.996& 0.998& 0.999& 1.000& 1.000& 1.000& 0.999& 0.998\\ 
0.986& 0.989& 0.992& 0.994& 0.996& 0.998& 0.999& 1.000& 1.000& 1.000& 0.999\\ 
0.982& 0.985& 0.989& 0.992& 0.994& 0.996& 0.998& 0.999& 1.000& 1.000& 1.000\\ 
0.977& 0.981& 0.985& 0.988& 0.991& 0.994& 0.996& 0.998& 0.999& 1.000& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}


==> Paper-Final Version/tabs/systematics_data_FV_Dphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_V \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_V $  & $\Delta_{F_V} $\\ \hline
0 &  -0.150466 &  0.0144033 \\ \hline 
0.1 &  -0.135916 &  0.0119914 \\ \hline 
0.2 &  -0.123034 &  0.0114497 \\ \hline 
0.3 &  -0.111365 &  0.0119456 \\ \hline 
0.4 &  -0.100606 &  0.0132415 \\ \hline 
0.5 &  -0.0905481 &  0.0152892 \\ \hline 
0.6 &  -0.0810413 &  0.0180286 \\ \hline 
0.7 &  -0.071976 &  0.0213636 \\ \hline 
0.8 &  -0.0632697 &  0.0251904 \\ \hline 
0.9 &  -0.0548596 &  0.0294171 \\ \hline 
1 &  -0.0466964 &  0.0339692 \\ \hline 
\end{tabular}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 0.925& 0.749& 0.552& 0.377& 0.239& 0.140& 0.072& 0.027& -0.003& -0.023\\ 
0.925& 1.000& 0.941& 0.807& 0.647& 0.494& 0.364& 0.263& 0.187& 0.130& 0.087\\ 
0.749& 0.941& 1.000& 0.956& 0.851& 0.721& 0.596& 0.488& 0.401& 0.331& 0.276\\ 
0.552& 0.807& 0.956& 1.000& 0.966& 0.885& 0.789& 0.696& 0.615& 0.547& 0.492\\ 
0.377& 0.647& 0.851& 0.966& 1.000& 0.975& 0.918& 0.852& 0.788& 0.732& 0.684\\ 
0.239& 0.494& 0.721& 0.885& 0.975& 1.000& 0.983& 0.946& 0.904& 0.862& 0.824\\ 
0.140& 0.364& 0.596& 0.789& 0.918& 0.983& 1.000& 0.989& 0.966& 0.939& 0.913\\ 
0.072& 0.263& 0.488& 0.696& 0.852& 0.946& 0.989& 1.000& 0.993& 0.979& 0.962\\ 
0.027& 0.187& 0.401& 0.615& 0.788& 0.904& 0.966& 0.993& 1.000& 0.996& 0.987\\ 
-0.003& 0.130& 0.331& 0.547& 0.732& 0.862& 0.939& 0.979& 0.996& 1.000& 0.997\\ 
-0.023& 0.087& 0.276& 0.492& 0.684& 0.824& 0.913& 0.962& 0.987& 0.997& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}


==> Paper-Final Version/tabs/systematics_data_FV_Dsphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_V \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_V $  & $\Delta_{F_V} $\\ \hline
0 &  -0.120018 &  0.0155225 \\ \hline 
0.1 &  -0.0989568 &  0.0117214 \\ \hline 
0.2 &  -0.0824261 &  0.00951697 \\ \hline 
0.3 &  -0.0684115 &  0.00783577 \\ \hline 
0.4 &  -0.05594 &  0.00806476 \\ \hline 
0.5 &  -0.0444834 &  0.0110619 \\ \hline 
0.6 &  -0.03373 &  0.0158477 \\ \hline 
0.7 &  -0.0234841 &  0.0215682 \\ \hline 
0.8 &  -0.0136163 &  0.0278383 \\ \hline 
0.9 &  -0.00403801 &  0.0344741 \\ \hline 
1 &  0.00531392 &  0.0413737 \\ \hline 
\end{tabular}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 0.933& 0.886& 0.898& 0.782& 0.543& 0.379& 0.288& 0.236& 0.205& 0.184\\ 
0.933& 1.000& 0.989& 0.935& 0.667& 0.317& 0.107& -0.004& -0.066& -0.103& -0.127\\ 
0.886& 0.989& 1.000& 0.955& 0.679& 0.314& 0.093& -0.024& -0.090& -0.130& -0.157\\ 
0.898& 0.935& 0.955& 1.000& 0.862& 0.571& 0.369& 0.255& 0.188& 0.147& 0.119\\ 
0.782& 0.667& 0.679& 0.862& 1.000& 0.908& 0.787& 0.707& 0.656& 0.623& 0.600\\ 
0.543& 0.317& 0.314& 0.571& 0.908& 1.000& 0.973& 0.938& 0.912& 0.893& 0.879\\ 
0.379& 0.107& 0.093& 0.369& 0.787& 0.973& 1.000& 0.993& 0.982& 0.972& 0.965\\ 
0.288& -0.004& -0.024& 0.255& 0.707& 0.938& 0.993& 1.000& 0.998& 0.993& 0.990\\ 
0.236& -0.066& -0.090& 0.188& 0.656& 0.912& 0.982& 0.998& 1.000& 0.999& 0.997\\ 
0.205& -0.103& -0.130& 0.147& 0.623& 0.893& 0.972& 0.993& 0.999& 1.000& 1.000\\ 
0.184& -0.127& -0.157& 0.119& 0.600& 0.879& 0.965& 0.990& 0.997& 1.000& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}


==> Paper-Final Version/tabs/systematics_data_FV_Kphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_V \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_V $  & $\Delta_{F_V} $\\ \hline
0 &  0.12439 &  0.00960998 \\ \hline 
0.1 &  0.121998 &  0.00891388 \\ \hline 
0.2 &  0.119606 &  0.00828371 \\ \hline 
0.3 &  0.117214 &  0.0077356 \\ \hline 
0.4 &  0.114821 &  0.0072881 \\ \hline 
0.5 &  0.112429 &  0.00696062 \\ \hline 
0.6 &  0.110037 &  0.00677062 \\ \hline 
0.7 &  0.107645 &  0.00672974 \\ \hline 
0.8 &  0.105253 &  0.00684066 \\ \hline 
0.9 &  0.102861 &  0.00709626 \\ \hline 
1 &  0.100469 &  0.00748173 \\ \hline 
\end{tabular}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 0.997& 0.985& 0.961& 0.921& 0.860& 0.777& 0.674& 0.558& 0.435& 0.316\\ 
0.997& 1.000& 0.996& 0.980& 0.949& 0.898& 0.825& 0.731& 0.622& 0.506& 0.391\\ 
0.985& 0.996& 1.000& 0.994& 0.974& 0.935& 0.874& 0.791& 0.692& 0.583& 0.474\\ 
0.961& 0.980& 0.994& 1.000& 0.993& 0.967& 0.921& 0.852& 0.765& 0.666& 0.565\\ 
0.921& 0.949& 0.974& 0.993& 1.000& 0.991& 0.961& 0.909& 0.837& 0.752& 0.661\\ 
0.860& 0.898& 0.935& 0.967& 0.991& 1.000& 0.989& 0.957& 0.903& 0.834& 0.756\\ 
0.777& 0.825& 0.874& 0.921& 0.961& 0.989& 1.000& 0.989& 0.956& 0.905& 0.843\\ 
0.674& 0.731& 0.791& 0.852& 0.909& 0.957& 0.989& 1.000& 0.989& 0.958& 0.914\\ 
0.558& 0.622& 0.692& 0.765& 0.837& 0.903& 0.956& 0.989& 1.000& 0.990& 0.964\\ 
0.435& 0.506& 0.583& 0.666& 0.752& 0.834& 0.905& 0.958& 0.990& 1.000& 0.992\\ 
0.316& 0.391& 0.474& 0.565& 0.661& 0.756& 0.843& 0.914& 0.964& 0.992& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}


==> Paper-Final Version/tabs/systematics_data_FV_Piphys.tex <==
\begin{eqnarray} && \qquad \qquad \qquad \qquad   \qquad \qquad \qquad \qquad \qquad   F_V \quad {\rm Correlation} \quad  {\rm  Matrix} \nonumber \\ &&\footnotesize{
\begin{tabular}{|c|c|c|}
\hline
 $x_\gamma$  & $F_V $  & $\Delta_{F_V} $\\ \hline
0 &  0.0233352 &  0.00214581 \\ \hline 
0.1 &  0.023309 &  0.0021304 \\ \hline 
0.2 &  0.0232828 &  0.00211523 \\ \hline 
0.3 &  0.0232566 &  0.00210031 \\ \hline 
0.4 &  0.0232303 &  0.00208563 \\ \hline 
0.5 &  0.0232041 &  0.00207121 \\ \hline 
0.6 &  0.0231779 &  0.00205705 \\ \hline 
0.7 &  0.0231517 &  0.00204315 \\ \hline 
0.8 &  0.0231254 &  0.00202952 \\ \hline 
0.9 &  0.0230992 &  0.00201617 \\ \hline 
1 &  0.023073 &  0.0020031 \\ \hline 
\end{tabular}
\vspace{0.4in}
\quad \left(\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}1.000& 1.000& 1.000& 0.999& 0.999& 0.999& 0.998& 0.997& 0.996& 0.995& 0.994\\ 
1.000& 1.000& 1.000& 1.000& 0.999& 0.999& 0.998& 0.998& 0.997& 0.996& 0.995\\ 
1.000& 1.000& 1.000& 1.000& 1.000& 0.999& 0.999& 0.998& 0.998& 0.997& 0.996\\ 
0.999& 1.000& 1.000& 1.000& 1.000& 1.000& 0.999& 0.999& 0.998& 0.998& 0.997\\ 
0.999& 0.999& 1.000& 1.000& 1.000& 1.000& 1.000& 0.999& 0.999& 0.998& 0.998\\ 
0.999& 0.999& 0.999& 1.000& 1.000& 1.000& 1.000& 1.000& 0.999& 0.999& 0.998\\ 
0.998& 0.998& 0.999& 0.999& 1.000& 1.000& 1.000& 1.000& 1.000& 0.999& 0.999\\ 
0.997& 0.998& 0.998& 0.999& 0.999& 1.000& 1.000& 1.000& 1.000& 1.000& 0.999\\ 
0.996& 0.997& 0.998& 0.998& 0.999& 0.999& 1.000& 1.000& 1.000& 1.000& 1.000\\ 
0.995& 0.996& 0.997& 0.998& 0.998& 0.999& 0.999& 1.000& 1.000& 1.000& 1.000\\ 
0.994& 0.995& 0.996& 0.997& 0.998& 0.998& 0.999& 0.999& 1.000& 1.000& 1.000\\ 
\end{tabular}\right) \nonumber
  }\end{eqnarray}

